InfeRE: Step-by-Step Regex Generation via Chain of Inference

Automatically generating regular expressions (abbrev. regexes) from natural language description (NL2RE) has been an emerging research area. Prior studies treat regex as a linear sequence of tokens and generate the final expressions autoregressively in a single pass. They did not take into account the step-by-step internal text-matching processes behind the final results. This significantly hinders the efficacy and interpretability of regex generation by neural language models. In this paper, we propose a new paradigm called InfeRE, which decomposes the generation of regexes into chains of step-by-step inference. To enhance the robustness, we introduce a self-consistency decoding mechanism that ensembles multiple outputs sampled from different models. We evaluate InfeRE on two publicly available datasets, NL-RX-Turk and KB13, and compare the results with state-of-the-art approaches and the popular tree-based generation approach TRANX. Experimental results show that InfeRE substantially outperforms previous baselines, yielding 16.3% and 14.7% improvement in DFA@5 accuracy on two datasets, respectively. Particularly, InfeRE outperforms the popular tree-based generation approach by 18.1% and 11.3% on both datasets, respectively, in terms of DFA@5 accuracy.

==> tables/motivation.tex <==
\begin{table}
\caption{A motivation example of step-by-step regex generation. We decompose the generation of a regex into 5 steps, with the step description (middle) and the internal results (right).
The bottom half shows the order for generating each token according to the decomposition. We use integer numbers to indicate the order. It is shown that the generation does not follow a left-to-right order as the conventional sequence-to-sequence model assumes. For example, the first left bracket is emitted lastly when we consider the \emph{and} operator.
}
\label{motivateexample}
\centering
\small
\scalebox{0.91}{
\begin{tabular}{c|l|l}
\toprule
\multicolumn{3}{l}{\textbf{Q}: lines starting with a lower-case letter and ending with vowel}  \\
\bottomrule
 Step 1  & lower-case letter & [a-z]    \\
\hline
 Step 2 & starts with & [a-z](.*)\\
\hline
 Step 3 & vowel letter & [AEIOUaeiou] \\
\hline
 Step 4 & end with &(.*)[AEIOUaeiou] \\
\hline
 Step 5 & and & (([a-z])(.*))\&((.*)([AEIOUaeiou]))\\
%\bottomrule
%  & What [1] is [1] the [2] reason [3] of [2] World [4] War [4] II [5] ? \\
\bottomrule
\end{tabular}}

\scalebox{0.91}{
\begin{tabular}{l}
  ~~~~~~~~~~~~~~~~~~~~$\Downarrow$\\
 \toprule
  \textbf{Generation Order by Autoregressive LMs}: \\
  \toprule
  ( ([a-z])(.*) )\&( (.*)( [AEIOUaeiou] )) \\
    \textcolor{blue}{$^{123456789........}$}\\
  \toprule
  \textbf{Real Order of Text-Matching Processes}: \\
  \toprule
  ( ([a-z]) (.*) )\&( (.*)( [AEIOUaeiou] ))\\
  \textcolor{red}{$^5$}\textcolor{blue}{$^2$}\textcolor{yellow}{$^{11111}$}\textcolor{blue}{$^{22222}$}  \textcolor{red}{$^{555}$} \textcolor{green}{$^{4444}$} \textcolor{cyan}{$^{33\;33\;3\;33\;3\;33\;3}$}\textcolor{green}{$^4$}\textcolor{red}{$^5$} \\
  %What\textcolor{red}{$^1$} is\textcolor{red}{$^1$} the\textcolor{red}{$^2$} reason\textcolor{red}{$^3$} of\textcolor{red}{$^2$} World\textcolor{red}{$^4$} War\textcolor{red}{$^4$} II\textcolor{red}{$^5$} ? \\
  \bottomrule
\end{tabular}
}

%\vspace{-2\baselineskip}
\end{table}

==> tables/motivation_ase23.tex <==
\begin{table}[t]
\caption{\small A motivation example of step-by-step regex generation. 
}
\label{motivateexample}
\centering
\small

\scalebox{0.91}{
\begin{tabular}{c|l|l}
\toprule
\multicolumn{3}{l}{\textbf{Q}: lines starting with a lower-case letter and ending with vowel}  \\
\bottomrule
 Step 1  & lower-case letter & [a-z]    \\
\hline
 Step 2 & starts with & [a-z](.*)\\
\hline
 Step 3 & vowel letter & [AEIOUaeiou] \\
\hline
 Step 4 & end with &(.*)[AEIOUaeiou] \\
\hline
 Step 5 & and & (([a-z])(.*))\&((.*)([AEIOUaeiou]))\\
%\bottomrule
%  & What [1] is [1] the [2] reason [3] of [2] World [4] War [4] II [5] ? \\
\bottomrule
\end{tabular}}

\scalebox{0.91}{
\begin{tabular}{l}
  ~~~~~~~~~~~~~~~~~~~~$\Downarrow$\\
 \toprule
  \textbf{Generation Order by Autoregressive LMs}: \\
  \toprule
  ( ([a-z])(.*) )\&( (.*)( [AEIOUaeiou] )) \\
    \textcolor{blue}{$^{1\;23456789........}$}\\
  \toprule
  \textbf{Real Order of Text-Matching Processes}: \\
  \toprule
  ( ([a-z]) (.*) )\&( (.*)( [AEIOUaeiou] ))\\
  \textcolor{red}{$^5$}\textcolor{blue}{$^2$}\textcolor{yellow}{$^{11111}$}\textcolor{blue}{$^{22222}$}  \textcolor{red}{$^{555}$} \textcolor{green}{$^{4444}$} \;\textcolor{cyan}{$^{33\;33\;3\;33\;3\;33\;3}$}\textcolor{green}{$^4$}\textcolor{red}{$^5$} \\
  %What\textcolor{red}{$^1$} is\textcolor{red}{$^1$} the\textcolor{red}{$^2$} reason\textcolor{red}{$^3$} of\textcolor{red}{$^2$} World\textcolor{red}{$^4$} War\textcolor{red}{$^4$} II\textcolor{red}{$^5$} ? \\
  \bottomrule
\end{tabular}
}

%\vspace{-2\baselineskip}
\end{table}

==> tables/motivation_zs.tex <==
\begin{table}[t]
\caption{\small A motivation example of step-by-step regex generation. 
}
\label{motivateexample}
\centering
\small

\begin{tabular}{l}
 \toprule
  \textbf{\textbf{Q}: lines starting with a lower-case letter and ending with vowel} \\
 \bottomrule
\end{tabular}
~~~~\\
~~~~\\
~~~~\\
\scalebox{0.91}{
\begin{tabular}{c|l|l}
\toprule
\multicolumn{3}{c}{\textbf{Intermediate Steps}}  \\
  \toprule
 Step 1  & lower-case letter & [a-z]    \\
\hline
 Step 2 & starts with & [a-z](.*)\\
\hline
 Step 3 & vowel letter & [AEIOUaeiou] \\
\hline
 Step 4 & end with &(.*)[AEIOUaeiou] \\
\hline
 Step 5 & and & (([a-z])(.*))\&((.*)([AEIOUaeiou]))\\
%\bottomrule
%  & What [1] is [1] the [2] reason [3] of [2] World [4] War [4] II [5] ? \\
\bottomrule
\end{tabular}}
~~~~\\
~~~~\\
~~~~\\
\scalebox{0.81}{
\begin{tabular}{ll}
  \toprule
  \makecell{\textbf{The Real Order of }\\ \textbf{Text-Matching Processes}}& 
  \makecell{\textbf{The Generation Order by }\\ \textbf{Autoregressive LMs}}\\
  \toprule
  \makecell{( ([a-z]) (.*) )\&( (.*)( [AEIOUaeiou] ))\\
  \textcolor{red}{$^5$}\textcolor{blue}{$^2$}\textcolor{orange}{$^{11111}$}\textcolor{blue}{$^{22222}$}  \textcolor{red}{$^{555}$} \textcolor{green}{$^{4444}$} \;\textcolor{cyan}{$^{33\;33\;3\;33\;3\;33\;3}$}\textcolor{green}{$^4$}\textcolor{red}{$^5$} \\}
  &
    \makecell[l]{( ([a-z])(.*) )\&( (.*)( [AEIOUaeiou] )) \\
    \textcolor{blue}{$^{1\;23456789........}$}}\\
  %What\textcolor{red}{$^1$} is\textcolor{red}{$^1$} the\textcolor{red}{$^2$} reason\textcolor{red}{$^3$} of\textcolor{red}{$^2$} World\textcolor{red}{$^4$} War\textcolor{red}{$^4$} II\textcolor{red}{$^5$} ? \\
  %What\textcolor{red}{$^1$} is\textcolor{red}{$^1$} the\textcolor{red}{$^2$} reason\textcolor{red}{$^3$} of\textcolor{red}{$^2$} World\textcolor{red}{$^4$} War\textcolor{red}{$^4$} II\textcolor{red}{$^5$} ? \\
  \bottomrule
\end{tabular}
}

%\vspace{-2\baselineskip}
\end{table}
